Sequential Keystroke Behavioral Biometrics for Mobile User Identification via Multi-view Deep Learning

With the rapid growth in smartphone usage, more organizations begin to focus on providing better services for mobile users. User identification can help these organizations to identify their customers and then cater services that have been customized for them. Currently, the use of cookies is the most common form to identify users. However, cookies are not easily transportable (e.g., when a user uses a different login account, cookies do not follow the user). This limitation motivates the need to use behavior biometric for user identification. In this paper, we propose DEEPSERVICE, a new technique that can identify mobile users based on user's keystroke information captured by a special keyboard or web browser. Our evaluation results indicate that DEEPSERVICE is highly accurate in identifying mobile users (over 93% accuracy). The technique is also efficient and only takes less than 1 ms to perform identification.

==> references.tex <==
@misc{china15,
 author = {China News},
 title = {{New Tricks for Fraudulent Message}},
 howpublished = 
 {{http://www.chinanews.com/life/2015/11-05/7607797.shtml}},
 month = {Nov},
 year = {2015},
}

@article{ruder2016overview,
  title={An overview of gradient descent optimization algorithms},
  author={Ruder, Sebastian},
  journal={arXiv preprint arXiv:1609.04747},
  year={2016}
}

@misc{trevor16loss,
 author = {Trevor Mogg},
 title = {{STUDY REVEALS AMERICANS LOST \$30 BILLION WORTH OF MOBILE PHONES LAST YEAR}},
 howpublished = 
 {{http://www.digitaltrends.com/mobile/study-reveals-americans-lost-30-billion-of-mobile-phones-last-year/}},
 month = {Mar},
 year = {2012},
}

@misc{idc16,
 author = {IDC Research},
 title = {{Smartphone Vendor Market Share, 2016}},
 howpublished = 
 {{http://www.idc.com/}},
 month = {Nov},
 year = {2016},
}

@misc{watson2015,
 author = {Secil Watson},
 title = {{Impostor Fraud: A Cyber Risk Management Challenge}},
 howpublished = {{http://www.treasuryandrisk.com/2015/05/05/impostor-fraud-a-cyber-risk-management-challenge?slreturn=1485885396}},
 month = {May},
 year = {2015},
}

@misc{nick2016passcode,
 author = {Nick Mediati},
 title = {{Pew survey shows 68 percent of US adults now own a smartphone}},
 howpublished = 
 {{http://www.pcworld.com/article/2999631/phones/pew-survey-shows-68-percent-of-americans-now-own-a-smartphone.html}},
 month = {Nov},
 year = {2015},
}

@misc{ethan2016passcode,
 author = {Ethan Wolff-Mann},
 title = {{It’s Not Hard to Fake a Fingerprint to Break into a Phone}},
 howpublished = 
 {{http://time.com/money/4315040/fingerprint-security-phone-hack-break/}},
 month = {May},
 year = {2016},
}

@misc{panda2016passcode,
 author = {Panda Security},
 title = {{75 million smartphones in the US don’t have their passwords set on}},
 howpublished = 
 {{http://www.pandasecurity.com/mediacenter/tips/smartphone-risk-dont-use-password/}},
 month = {Sep},
 year = {2015},
}

@misc{kate15passcode,
 author = {Kate Knibbs},
 title = {{Start Memorizing Your Six-Digit iPhone Passcode}},
 howpublished = 
 {{ http://gizmodo.com/start-memorizing-your-six-digit-iphone-passcode-1710072672}},
 month = {Sep},
 year = {2015},
}

@misc{kateknibbs15,
 author = {Kate Knibbs},
 title = {{Start Memorizing Your Six-Digit iPhone Passcode}},
 howpublished = 
 {{ http://gizmodo.com/start-memorizing-your-six-digit-iphone-passcode-1710072672}},
 month = {Sep},
 year = {2015},
}

@misc{daniel11passcode,
 author = {Daniel Amitay},
 title = {{Most Common iPhone Passcodes}},
 howpublished = 
 {{http://danielamitay.com/blog/2011/6/13/most-common-iphone-passcodes}},
 month = {Jun},
 year = {2011},
}
 
  @misc{statista16,
 author = {Statista Inc.},
 title = {{Number of smartphone users worldwide from 2014 to 2020 (in billions)}},
 howpublished = 
 {{ https://www.statista.com/statistics/330695/number-of-smartphone-users-worldwide/}},
 month = {November},
 year = {2016},
 }
 
 @inproceedings{femila2011biometric,
  title={Biometric system},
  author={Femila, M Daris and Irudhayaraj, A Anthony},
  booktitle={Electronics Computer Technology (ICECT), 2011 3rd International Conference on},
  volume={1},
  pages={152--156},
  year={2011},
  organization={IEEE}
}

@inproceedings{karlson2009can,
  title={Can i borrow your phone?: understanding concerns when sharing mobile phones},
  author={Karlson, Amy K and Brush, AJ and Schechter, Stuart},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={1647--1650},
  year={2009},
  organization={ACM}
}

@article{cai2011touchlogger,
  title={TouchLogger: Inferring Keystrokes on Touch Screen from Smartphone Motion.},
  author={Cai, Liang and Chen, Hao},
  journal={HotSec},
  volume={11},
  pages={9--9},
  year={2011}
}

@inproceedings{miluzzo2012tapprints,
  title={Tapprints: your finger taps have fingerprints},
  author={Miluzzo, Emiliano and Varshavsky, Alexander and Balakrishnan, Suhrid and Choudhury, Romit Roy},
  booktitle={Proceedings of the 10th international conference on Mobile systems, applications, and services},
  pages={323--336},
  year={2012},
  organization={ACM}
}

@inproceedings{owusu2012accessory,
  title={ACCessory: password inference using accelerometers on smartphones},
  author={Owusu, Emmanuel and Han, Jun and Das, Sauvik and Perrig, Adrian and Zhang, Joy},
  booktitle={Proceedings of the Twelfth Workshop on Mobile Computing Systems \& Applications},
  pages={9},
  year={2012},
  organization={ACM}
}

@inproceedings{xu2012taplogger,
  title={Taplogger: Inferring user inputs on smartphone touchscreens using on-board motion sensors},
  author={Xu, Zhi and Bai, Kun and Zhu, Sencun},
  booktitle={Proceedings of the fifth ACM conference on Security and Privacy in Wireless and Mobile Networks},
  pages={113--124},
  year={2012},
  organization={ACM}
}

@article{aviv2010smudge,
  title={Smudge Attacks on Smartphone Touch Screens.},
  author={Aviv, Adam J and Gibson, Katherine and Mossop, Evan and Blaze, Matt and Smith, Jonathan M},
  journal={WOOT},
  volume={10},
  pages={1--7},
  year={2010}
}

@inproceedings{bo2013you,
  title={You're driving and texting: detecting drivers using personal smart phones by leveraging inertial sensors},
  author={Bo, Cheng and Jian, Xuesi and Li, Xiang-Yang and Mao, Xufei and Wang, Yu and Li, Fan},
  booktitle={Proceedings of the 19th annual international conference on Mobile computing \& networking},
  pages={199--202},
  year={2013},
  organization={ACM}
}

@inproceedings{bo2014continuous,
  title={Continuous user identification via touch and movement behavioral biometrics},
  author={Bo, Cheng and Zhang, Lan and Jung, Taeho and Han, Junze and Li, Xiang-Yang and Wang, Yu},
  booktitle={2014 IEEE 33rd International Performance Computing and Communications Conference (IPCCC)},
  pages={1--8},
  year={2014},
  organization={IEEE}
}

@inproceedings{zheng2014you,
  title={You are how you touch: User verification on smartphones via tapping behaviors},
  author={Zheng, Nan and Bai, Kun and Huang, Hai and Wang, Haining},
  booktitle={2014 IEEE 22nd International Conference on Network Protocols},
  pages={221--232},
  year={2014},
  organization={IEEE}
}

@article{burges1998tutorial,
  title={A tutorial on support vector machines for pattern recognition},
  author={Burges, Christopher JC},
  journal={Data mining and knowledge discovery},
  volume={2},
  number={2},
  pages={121--167},
  year={1998},
  publisher={Springer}
}

@article{quinlan1986induction,
  title={Induction of decision trees},
  author={Quinlan, J. Ross},
  journal={Machine learning},
  volume={1},
  number={1},
  pages={81--106},
  year={1986},
  publisher={Springer}
}

@article{breiman2001random,
  title={Random forests},
  author={Breiman, Leo},
  journal={Machine learning},
  volume={45},
  number={1},
  pages={5--32},
  year={2001},
  publisher={Springer}
}

@article{chen2016xgboost,
  title={Xgboost: A scalable tree boosting system},
  author={Chen, Tianqi and Guestrin, Carlos},
  journal={arXiv preprint arXiv:1603.02754},
  year={2016}
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}

@article{chung2014empirical,
  title={Empirical evaluation of gated recurrent neural networks on sequence modeling},
  author={Chung, Junyoung and Gulcehre, Caglar and Cho, KyungHyun and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1412.3555},
  year={2014}
}


@article{banerjee2012biometric,
  title={Biometric authentication and identification using keystroke dynamics: A survey},
  author={Banerjee, Salil P and Woodard, Damon L},
  journal={Journal of Pattern Recognition Research},
  volume={7},
  number={1},
  pages={116--139},
  year={2012},
  publisher={Citeseer}
}

@inproceedings{goh2003computation,
  title={Computation of cryptographic keys from face biometrics},
  author={Goh, Alwyn and Ngo, David CL},
  booktitle={IFIP International Conference on Communications and Multimedia Security},
  pages={1--13},
  year={2003},
  organization={Springer}
}

@inproceedings{prokoski2000history,
  title={History, current status, and future of infrared identification},
  author={Prokoski, Francine},
  booktitle={Computer Vision Beyond the Visible Spectrum: Methods and Applications, 2000. Proceedings. IEEE Workshop on},
  pages={5--14},
  year={2000},
  organization={IEEE}
}

@inproceedings{de2001iris,
  title={Iris recognition for biometric identification using dyadic wavelet transform zero-crossing},
  author={de Martin-Roche, D and Sanchez-Avila, Carmen and Sanchez-Reillo, Raul},
  booktitle={Security Technology, 2001 IEEE 35th International Carnahan Conference on},
  pages={272--277},
  year={2001},
  organization={IEEE}
}

@inproceedings{messerman2011continuous,
  title={Continuous and non-intrusive identity verification in real-time environments based on free-text keystroke dynamics},
  author={Messerman, Arik and Mustafi{\'c}, Tarik and Camtepe, Seyit Ahmet and Albayrak, Sahin},
  booktitle={Biometrics (IJCB), 2011 International Joint Conference on},
  pages={1--8},
  year={2011},
  organization={IEEE}
}

@inproceedings{de2012touch,
  title={Touch me once and i know it's you!: implicit authentication based on touch screen patterns},
  author={De Luca, Alexander and Hang, Alina and Brudy, Frederik and Lindner, Christian and Hussmann, Heinrich},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={987--996},
  year={2012},
  organization={ACM}
}

@article{seo2012novel,
  title={A novel biometric identification based on a user's input pattern analysis for intelligent mobile devices},
  author={Seo, Hojin and Kim, Eunjin and Kim, Huy Kang},
  journal={International Journal of Advanced Robotic Systems},
  volume={9},
  number={2},
  pages={46},
  year={2012},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{frank2013touchalytics,
  title={Touchalytics: On the applicability of touchscreen input as a behavioral biometric for continuous authentication},
  author={Frank, Mario and Biedert, Ralf and Ma, Eugene and Martinovic, Ivan and Song, Dawn},
  journal={IEEE transactions on information forensics and security},
  volume={8},
  number={1},
  pages={136--148},
  year={2013},
  publisher={IEEE}
}

@inproceedings{feng2012continuous,
  title={Continuous mobile authentication using touchscreen gestures},
  author={Feng, Tao and Liu, Ziyi and Kwon, Kyeong-An and Shi, Weidong and Carbunar, Bogdan and Jiang, Yifei and Nguyen, Nhung},
  booktitle={Homeland Security (HST), 2012 IEEE Conference on Technologies for},
  pages={451--456},
  year={2012},
  organization={IEEE}
}

@article{niinuma2010soft,
  title={Soft biometric traits for continuous user authentication},
  author={Niinuma, Koichiro and Park, Unsang and Jain, Anil K},
  journal={IEEE Transactions on information forensics and security},
  volume={5},
  number={4},
  pages={771--780},
  year={2010},
  publisher={IEEE}
}

@inproceedings{shi2011senguard,
  title={Senguard: Passive user identification on smartphones using multiple sensors},
  author={Shi, Weidong and Yang, Jun and Jiang, Yifei and Yang, Feng and Xiong, Yingen},
  booktitle={Wireless and Mobile Computing, Networking and Communications (WiMob), 2011 IEEE 7th International Conference on},
  pages={141--148},
  year={2011},
  organization={IEEE}
}

@inproceedings{zhao2013continuous,
  title={Continuous mobile authentication using a novel graphic touch gesture feature},
  author={Zhao, Xi and Feng, Tao and Shi, Weidong},
  booktitle={Biometrics: Theory, Applications and Systems (BTAS), 2013 IEEE Sixth International Conference on},
  pages={1--6},
  year={2013},
  organization={IEEE}
}

@article{ma2003personal,
  title={Personal identification based on iris texture analysis},
  author={Ma, Li and Tan, Tieniu and Wang, Yunhong and Zhang, Dexin},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={25},
  number={12},
  pages={1519--1533},
  year={2003},
  publisher={IEEE}
}

@inproceedings{cao2016multi,
  title={Multi-view Machines},
  author={Cao, Bokai and Zhou, Hucheng and Li, Guoqiang and Yu, Philip S.},
  booktitle={Proceedings of ACM International Conference on Web Search and Data Mining (WSDM)},
  year={2016}
}

@inproceedings{lu2017multilinear,
  title={Multilinear Factorization Machines for Multi-Task Multi-View Learning},
  author={Lu, Chun-Ta and He, Lifang and Shao, Weixiang and Cao, Bokai and Yu, Philip S.},
  booktitle={Proceedings of ACM International Conference on Web Search and Data Mining (WSDM)},
  year={2017}
}


@article{sun2016sigpid,
  title={SigPID: Significant Permission Identification for Android Malware Detection},
  author={Sun, Lichao and Li, Zhiqiang and Yan, Qiben and Srisa-an, Witawas},
  year={2016},
  organization={IEEE}
}

@inproceedings{arp2014drebin,
  title={DREBIN: Effective and Explainable Detection of Android Malware in Your Pocket.},
  author={Arp, Daniel and Spreitzenbarth, Michael and Hubner, Malte and Gascon, Hugo and Rieck, Konrad and Siemens, CERT},
  booktitle={NDSS},
  year={2014}
}

@article{shao2016online,
  title={Online Multi-view Clustering with Incomplete Views},
  author={Shao, Weixiang and He, Lifang and Lu, Chun-Ta and Yu, Philip S},
  journal={arXiv preprint arXiv:1611.00481},
  year={2016}
}

@inproceedings{cao2014tensor,
  title={Tensor-based multi-view feature selection with applications to brain diseases},
  author={Cao, Bokai and He, Lifang and Kong, Xiangnan and Philip, S Yu and Hao, Zhifeng and Ragin, Ann B},
  booktitle={Data Mining (ICDM), 2014 IEEE International Conference on},
  pages={40--49},
  year={2014},
  organization={IEEE}
}

@inproceedings{alghamdi2015dynamic,
  title={Dynamic User Verification Using Touch Keystroke Based on Medians Vector Proximity},
  author={Alghamdi, Shatha J and Elrefaei, Lamiaa A},
  booktitle={Computational Intelligence, Communication Systems and Networks (CICSyN), 2015 7th International Conference on},
  pages={121--126},
  year={2015},
  organization={IEEE}
}

@inproceedings{murmuria2015continuous,
  title={Continuous authentication on mobile devices using power consumption, touch gestures and physical movement of users},
  author={Murmuria, Rahul and Stavrou, Angelos and Barbar{\'a}, Daniel and Fleck, Dan},
  booktitle={International Workshop on Recent Advances in Intrusion Detection},
  pages={405--424},
  year={2015},
  organization={Springer}
}

@article{li2016privacy,
  title={Privacy protection for preventing data over-collection in smart city},
  author={Li, Yibin and Dai, Wenyun and Ming, Zhong and Qiu, Meikang},
  journal={IEEE Transactions on Computers},
  volume={65},
  number={5},
  pages={1339--1350},
  year={2016},
  publisher={IEEE}
}

@article{sakamoto2014droidtrack,
  title={Droidtrack: Tracking and visualizing information diffusion for preventing information leakage on android},
  author={Sakamoto, Shunya and Okuda, Kenji and Nakatsuka, Ryo and Yamauchi, Toshihiro},
  journal={Journal of Internet Services and Information Security (JISIS)},
  volume={4},
  number={2},
  pages={55--69},
  year={2014}
}

@inproceedings{menon2013statistical,
  title={On the Statistical Consistency of Algorithms for Binary Classification under Class Imbalance.},
  author={Menon, Aditya Krishna and Narasimhan, Harikrishna and Agarwal, Shivani and Chawla, Sanjay},
  booktitle={ICML (3)},
  pages={603--611},
  year={2013}
}

@inproceedings{kennedy2009learning,
  title={Learning without default: A study of one-class classification and the low-default portfolio problem},
  author={Kennedy, Kenneth and Mac Namee, Brian and Delany, Sarah Jane},
  booktitle={Irish Conference on Artificial Intelligence and Cognitive Science},
  pages={174--187},
  year={2009},
  organization={Springer}
}

@inproceedings{kwapisz2010cell,
  title={Cell phone-based biometric identification},
  author={Kwapisz, Jennifer R and Weiss, Gary M and Moore, Samuel A},
  booktitle={Biometrics: Theory Applications and Systems (BTAS), 2010 Fourth IEEE International Conference on},
  pages={1--7},
  year={2010},
  organization={IEEE}
}

@inproceedings{abramson2013associative,
  title={Associative patterns of web browsing behavior},
  author={Abramson, Myriam and Gore, Shantanu},
  booktitle={2013 AAAI Fall Symposium Series},
  year={2013}
}

@inproceedings{zhang2014mfingerprint,
  title={Mfingerprint: Privacy-preserving user modeling with multimodal mobile device footprints},
  author={Zhang, Haipeng and Yan, Zhixian and Yang, Jun and Tapia, Emmanuel Munguia and Crandall, David J},
  booktitle={International Conference on Social Computing, Behavioral-Cultural Modeling, and Prediction},
  pages={195--203},
  year={2014},
  organization={Springer}
}

@misc{chollet2015keras,
  title={Keras},
  author={Chollet, Fran\c{c}ois and others},
  year={2015},
  publisher={GitHub},
  howpublished={\url{https://github.com/fchollet/keras}},
}

@article{scikit-learn,
 title={Scikit-learn: Machine Learning in {P}ython},
 author={Pedregosa, F. and Varoquaux, G. and Gramfort, A. and Michel, V.
         and Thirion, B. and Grisel, O. and Blondel, M. and Prettenhofer, P.
         and Weiss, R. and Dubourg, V. and Vanderplas, J. and Passos, A. and
         Cournapeau, D. and Brucher, M. and Perrot, M. and Duchesnay, E.},
 journal={Journal of Machine Learning Research},
 volume={12},
 pages={2825--2830},
 year={2011}
}

@inproceedings{he2014dusk,
  title={Dusk: A dual structure-preserving kernel for supervised tensor learning with applications to neuroimages},
  author={He, Lifang and Kong, Xiangnan and Yu, Philip S and Yang, Xiaowei and Ragin, Ann B and Hao, Zhifeng},
  booktitle={Proceedings of the 2014 SIAM International Conference on Data Mining},
  pages={127--135},
  year={2014},
  organization={SIAM}
}

@inproceedings{cao2017t,
  title={t-BNE: Tensor-based Brain Network Embedding},
  author={Cao, Bokai and He, Lifang and Wei, Xiaokai and Xing, Mengqi and Yu, Philip S and Klumpp, Heide and Leow, Alex D},
  organization={SIAM}
}  

@inproceedings{shao2015clustering,
  title={Clustering on Multi-source Incomplete Data via Tensor Modeling and Factorization.},
  author={Shao, Weixiang and He, Lifang and Philip, S Yu}
}

@inproceedings{he2017kernel,
  title={Kernelized Support Tensor Machines},
  author={He, Lifang and Lu, Chun-Ta and Ma, Guixiang and Wang, Shen and Shen, Linlin and Yu, Philip S. and Ragin, Ann B.},
  booktitle={Proceedings of the 34th International Conference on Machine Learning},
  year={2017}
}

@inproceedings{he2017multi,
  title={Multi-way Multi-level Kernel Modeling for Neuroimaging Classification},
  author={He, Lifang and Lu, Chun-Ta and Ding, Hao and Wang, Shen and Shen, Linlin and Yu, Philip S. and Ragin, Ann B.},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year={2017}
}
